Does Mapo Tofu Contain Coffee? Probing LLMs for Food-related Cultural Knowledge

Recent studies have highlighted the presence of cultural biases in Large Language Models (LLMs), yet often lack a robust methodology to dissect these phenomena comprehensively. Our work aims to bridge this gap by delving into the Food domain, a universally relevant yet culturally diverse aspect of human life. We introduce FmLAMA, a multilingual dataset centered on food-related cultural facts and variations in food practices. We analyze LLMs across various architectures and configurations, evaluating their performance in both monolingual and multilingual settings. By leveraging templates in six different languages, we investigate how LLMs interact with language-specific and cultural knowledge. Our findings reveal that (1) LLMs demonstrate a pronounced bias towards food knowledge prevalent in the United States; (2) Incorporating relevant cultural context significantly improves LLMs' ability to access cultural knowledge; (3) The efficacy of LLMs in capturing cultural nuances is highly dependent on the interplay between the probing language, the specific model architecture, and the cultural context in question. This research underscores the complexity of integrating cultural understanding into LLMs and emphasizes the importance of culturally diverse datasets to mitigate biases and enhance model performance across different cultural domains.

==> content/Hebrew_results.tex <==


\begin{table*}[t]
  \begin{subtable}{1\linewidth}
    \centering
    \scalebox{0.8}{
    \begin{tabular}{@{}lr|rrrrr|r@{}}
\toprule
\textbf{Origin}  & \textbf{Count} & \textbf{mB}                            & \textbf{mT5}                           & \textbf{Qwen2}                          & \textbf{Llama2}                        & \textbf{Llama3}                         & \textbf{Average} \\ \midrule
\textbf{Italy}   & 59 (18.6\%)    & 4.18±2.54                              & 4.30±1.49                              & 7.78±2.37                               & 3.97±1.47                              & 6.29±3.14                               & 5.30             \\
\textbf{U.S.}    & 67 (21.1\%)    & 8.62±7.22                              & \underline{8.13±2.02} & 9.09±4.52                               & 3.62±0.81                              & 10.17±4.44                              & 7.93             \\
\textbf{Turkey}  & 12 (3.9\%)     & \underline{8.99±8.65} & 6.33±4.01                              & 9.21±5.92                               & 2.93±1.18                              & \underline{10.68±6.33} & 7.63             \\
\textbf{Japan}   & 19 (6.0\%)     & 6.69±5.23                              & 5.99±3.64                              & 6.60±4.19                               & \underline{6.92±3.85} & 4.39±3.12                               & 6.12             \\
\textbf{France}  & 65 (20.5\%)    & 5.43±3.01                              & 4.54±0.92                              & 6.40±2.74                               & 2.72±0.54                              & 5.50±1.47                               & 4.92             \\
\textbf{U.K.}    & 23 (7.3\%)     & \textbf{9.43±6.79}    & 6.95±2.26                              & 9.79±5.06                               & 3.97±2.49                              & 10.08±5.66                              & 8.04             \\
\textbf{Mexico}  & 11 (3.5\%)     & 2.22±0.75                              & 2.26±0.74                              & 4.33±2.44                               & 2.87±1.99                              & 2.14±2.01                               & 2.76             \\
\textbf{India}   & 18 (5.7\%)     & 8.12±3.72                              & 3.31±1.07                              & 2.80±2.77                               & 3.26±1.95                              & 4.73±2.46                               & 4.44             \\
\textbf{Germany} & 11 (3.5\%)     & 7.57±5.98                              & \textbf{14.84±6.23}   & 8.59±3.46                               & 5.92±1.83                              & 9.38±5.42                               & 9.26             \\
\textbf{China}   & 9 (2.8\%)      & 3.61±3.34                              & 2.12±0.78                              & 3.75±3.62                               & 1.64±1.29                              & 4.05±1.62                               & 3.03             \\
\textbf{Iran}    & 6 (1.9\%)      & 8.58±5.37                              & 5.05±2.90                              & \textbf{19.40±9.90}    & 2.95±0.57                              & \textbf{20.63±10.96}   & 11.32            \\
\textbf{Greece}  & 6 (1.9\%)      & 2.76±0.60                              & 4.31±0.49                              & \underline{12.96±9.55} & \textbf{7.67±2.85}    & 3.34±2.19                               & 6.21             \\
\textbf{Spain}   & 7 (2.2\%)      & 4.58±1.81                              & 7.02±1.87                              & 3.86±1.66                               & 4.04±1.62                              & 2.82±1.26                               & 4.46             \\
\textbf{Russia}  & 4 (1.3\%)      & 4.31±3.65                              & 3.35±0.07                              & 2.10±0.28                               & 2.56±0.46                              & 2.56±0.44                               & 2.98             \\ \midrule
\textbf{ALL}     & 317 (100\%)    & 6.41±4.30                              & 5.77±1.59                              & 7.57±2.66                               & 3.74±0.85                              & 7.17±2.63                               & 6.13             \\ \bottomrule
\end{tabular}
}
    \caption{Performance results evaluated on \textbf{mAP} (\%).}
  \end{subtable}
  
  \medskip % 适当的垂直间距
  
  \begin{subtable}{1\linewidth}
    \centering
    \scalebox{0.8}{
\begin{tabular}{@{}l|rrrrr|r@{}}
\toprule
\textbf{Origin}  & \textbf{mB}                              & \textbf{mT5}                             & \textbf{Qwen2}                           & \textbf{Llama2}                          & \textbf{Llama3}                          & \textbf{Average} \\ \midrule
\textbf{Italy}   & 0.3102±0.03                              & 0.3320±0.03                              & 0.3197±0.03                              & 0.2973±0.04                              & 0.3265±0.05                              & 0.3171           \\
\textbf{U.S.}    & 0.3435±0.06                              & 0.3626±0.03                              & 0.3524±0.03                              & 0.3042±0.03                              & 0.3517±0.04                              & 0.3429           \\
\textbf{Turkey}  & 0.2976±0.06                              & 0.3225±0.05                              & 0.3110±0.04                              & 0.2621±0.05                              & 0.3296±0.10                              & 0.3046           \\
\textbf{Japan}   & 0.3134±0.05                              & 0.3167±0.04                              & 0.3114±0.05                              & 0.2839±0.03                              & 0.2899±0.02                              & 0.3031           \\
\textbf{France}  & 0.3082±0.03                              & 0.3509±0.04                              & 0.3334±0.02                              & 0.2838±0.04                              & 0.3134±0.03                              & 0.3179           \\
\textbf{U.K.}    & 0.3400±0.06                              & 0.3418±0.04                              & 0.3414±0.04                              & 0.2930±0.02                              & 0.3167±0.06                              & 0.3266           \\
\textbf{Mexico}  & 0.2959±0.05                              & \underline\{0.3829±0.06\} & 0.3420±0.06                              & 0.2847±0.06                              & 0.2865±0.04                              & 0.3184           \\
\textbf{India}   & \textbf\{0.3614±0.05\}    & 0.3437±0.06                              & 0.3354±0.01                              & 0.3133±0.04                              & 0.3192±0.05                              & 0.3346           \\
\textbf{Germany} & \underline\{0.3595±0.04\} & 0.3763±0.02                              & \underline\{0.3756±0.03\} & \underline\{0.3339±0.05\} & \underline\{0.3586±0.06\} & 0.3608           \\
\textbf{China}   & 0.2863±0.03                              & 0.3131±0.06                              & 0.2714±0.06                              & 0.2683±0.03                              & 0.2432±0.04                              & 0.2765           \\
\textbf{Iran}    & 0.3435±0.05                              & 0.3521±0.07                              & \textbf\{0.4569±0.07\}    & 0.2902±0.02                              & \textbf\{0.4416±0.09\}    & 0.3769           \\
\textbf{Greece}  & 0.3014±0.02                              & 0.3423±0.02                              & 0.3722±0.08                              & 0.3332±0.03                              & 0.2951±0.04                              & 0.3288           \\
\textbf{Spain}   & 0.3493±0.03                              & \textbf\{0.4229±0.07\}    & 0.3547±0.02                              & \textbf\{0.3635±0.06\}    & 0.3260±0.03                              & 0.3633           \\
\textbf{Russia}  & 0.3276±0.03                              & 0.3748±0.06                              & 0.3319±0.04                              & 0.3308±0.01                              & 0.3179±0.04                              & 0.3366           \\ \midrule
\textbf{ALL}     & 0.3237±0.04                              & 0.3484±0.03                              & 0.3369±0.02                              & 0.2969±0.03                              & 0.3248±0.04                              & 0.3261           \\ \bottomrule
\end{tabular}
    
}
    \caption{Performance results evaluated on \textbf{mWS}.}
  \end{subtable}
  
  \caption{Probing performance comparison with \textbf{Hebrew} prompts and \textbf{\textsc{FmLAMA}-\textit{he}} sub-dataset. 
  % ``B/mB'' respectively represent abbreviations for BERT and mBERT, ``XR'' denotes XLM-RoBERTa, ``b/l'' stands for base/large and ``c/u'' stands for cased/uncased. \textbf{Bold} and \underline{underline} represent the best-performing and second-performing cultural group within the same model. The \textit{Pearson correlation coefficient} between mAP and mWS is 0.31 based on the results above.
  }
  \label{tab:he_without}
\end{table*}



==> table/language/English_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\begin{tabular}{@{}llrrrrrrrrrrrr@{}}
\toprule
\textbf{Origin}                  & \textbf{Metric} & \textbf{Bb-c} & \textbf{Bb-u} & \textbf{Bl-c} & \textbf{Bl-u} & \textbf{Rb} & \textbf{Rl} & \textbf{mB-c} & \textbf{mB-u} & \textbf{XRb} & \textbf{XRl} & \textbf{mT5} & \textbf{T5} \\ \midrule
\multirow{3}{*}{\textbf{U.S.}}   & P@1             & 23.53         & 26.47         & 32.35         & 29.41         & 0.00        & 0.00        & 11.76         & 23.53         & 0.00         & 0.00         & 14.71        & 14.71       \\
                                 & P@5             & 14.71         & 10.59         & 14.71         & 11.18         & 2.94        & 2.94        & 7.06          & 11.76         & 2.35         & 2.35         & 7.06         & 4.12        \\
                                 & mAP             & 28.79         & 24.92         & 30.89         & 27.29         & 3.01        & 3.09        & 15.54         & 20.17         & 4.56         & 4.52         & 14.90        & 12.51       \\ \midrule
\multirow{3}{*}{\textbf{France}} & P@1             & 6.45          & 12.90         & 12.90         & 14.52         & 0.00        & 0.00        & 9.68          & 16.13         & 0.00         & 0.00         & 8.06         & 9.68        \\
                                 & P@5             & 4.19          & 3.87          & 4.84          & 5.81          & 6.45        & 6.45        & 5.16          & 4.19          & 0.00         & 0.00         & 3.87         & 3.23        \\
                                 & mAP             & 8.16          & 9.67          & 13.73         & 12.25         & 5.31        & 5.28        & 9.98          & 11.12         & 3.87         & 3.83         & 5.82         & 6.83        \\ \midrule
\multirow{3}{*}{\textbf{Italy}}  & P@1             & 7.69          & 7.69          & 15.38         & 12.82         & 0.00        & 0.00        & 7.69          & 15.38         & 0.00         & 0.00         & 12.82        & 5.13        \\
                                 & P@5             & 3.08          & 3.59          & 6.67          & 5.13          & 4.10        & 4.10        & 5.64          & 7.69          & 0.00         & 0.00         & 5.13         & 2.56        \\
                                 & mAP             & 12.25         & 11.49         & 16.66         & 14.32         & 4.48        & 4.85        & 11.02         & 17.87         & 3.00         & 3.01         & 11.68        & 6.69        \\ \midrule
\multirow{3}{*}{\textbf{India}}  & P@1             & 15.38         & 23.08         & 15.38         & 7.69          & 0.00        & 0.00        & 7.69          & 7.69          & 0.00         & 0.00         & 7.69         & 7.69        \\
                                 & P@5             & 7.69          & 6.15          & 6.15          & 6.15          & 1.54        & 1.54        & 6.15          & 7.69          & 0.00         & 0.00         & 3.08         & 4.62        \\
                                 & mAP             & 25.51         & 26.12         & 23.13         & 16.89         & 3.03        & 2.95        & 15.07         & 20.29         & 1.96         & 2.00         & 15.92        & 11.04       \\ \midrule
\multirow{3}{*}{\textbf{Japan}}  & P@1             & 10.53         & 10.53         & 10.53         & 5.26          & 5.26        & 5.26        & 21.05         & 15.79         & 5.26         & 5.26         & 0.00         & 0.00        \\
                                 & P@5             & 5.26          & 5.26          & 7.37          & 8.42          & 1.05        & 1.05        & 5.26          & 5.26          & 1.05         & 1.05         & 2.11         & 0.00        \\
                                 & mAP             & 12.76         & 12.35         & 11.13         & 12.36         & 7.85        & 7.76        & 16.10         & 12.03         & 6.53         & 6.62         & 4.96         & 2.02        \\ \midrule
\multirow{3}{*}{\textbf{U.K.}}   & P@1             & 33.33         & 26.67         & 46.67         & 53.33         & 0.00        & 0.00        & 40.00         & 46.67         & 0.00         & 0.00         & 26.67        & 26.67       \\
                                 & P@5             & 14.67         & 10.67         & 17.33         & 17.33         & 6.67        & 6.67        & 14.67         & 14.67         & 1.33         & 1.33         & 9.33         & 9.33        \\
                                 & mAP             & 30.58         & 27.41         & 38.31         & 45.98         & 8.40        & 8.40        & 30.83         & 34.28         & 7.52         & 7.47         & 28.94        & 27.66       \\ \midrule
\multirow{3}{*}{\textbf{Spain}}  & P@1             & 10.00         & 10.00         & 10.00         & 10.00         & 0.00        & 0.00        & 10.00         & 20.00         & 0.00         & 0.00         & 0.00         & 10.00       \\
                                 & P@5             & 8.00          & 8.00          & 8.00          & 8.00          & 4.00        & 4.00        & 12.00         & 10.00         & 0.00         & 0.00         & 2.00         & 4.00        \\
                                 & mAP             & 14.86         & 12.87         & 21.20         & 19.63         & 3.30        & 3.83        & 20.30         & 24.03         & 3.11         & 3.10         & 5.18         & 12.03       \\ \midrule
\multirow{3}{*}{\textbf{China}}  & P@1             & 22.22         & 0.00          & 0.00          & 22.22         & 0.00        & 0.00        & 11.11         & 0.00          & 0.00         & 0.00         & 0.00         & 0.00        \\
                                 & P@5             & 8.89          & 6.67          & 6.67          & 13.33         & 0.00        & 0.00        & 6.67          & 4.44          & 0.00         & 0.00         & 4.44         & 4.44        \\
                                 & mAP             & 23.35         & 14.56         & 13.54         & 32.73         & 2.96        & 2.82        & 17.47         & 6.45          & 1.11         & 0.99         & 7.35         & 5.22        \\ \midrule
\multirow{3}{*}{\textbf{Turkey}} & P@1             & 23.53         & 23.53         & 23.53         & 5.88          & 0.00        & 0.00        & 29.41         & 29.41         & 0.00         & 0.00         & 11.76        & 5.88        \\
                                 & P@5             & 8.24          & 8.24          & 8.24          & 7.06          & 0.00        & 0.00        & 9.41          & 9.41          & 0.00         & 0.00         & 4.71         & 1.18        \\
                                 & mAP             & 18.57         & 20.39         & 20.33         & 13.90         & 2.69        & 2.71        & 23.83         & 25.40         & 1.90         & 1.90         & 11.82        & 8.75        \\ \midrule
\multirow{3}{*}{\textbf{Mexico}} & P@1             & 7.69          & 0.00          & 23.08         & 15.38         & 0.00        & 0.00        & 7.69          & 0.00          & 0.00         & 0.00         & 0.00         & 7.69        \\
                                 & P@5             & 7.69          & 9.23          & 6.15          & 9.23          & 1.54        & 1.54        & 4.62          & 3.08          & 1.54         & 1.54         & 3.08         & 1.54        \\
                                 & mAP             & 12.90         & 16.46         & 21.61         & 24.33         & 2.85        & 3.70        & 8.80          & 7.96          & 2.55         & 2.62         & 4.81         & 5.18        \\ \midrule
\multirow{3}{*}{\textbf{Others}} & P@1             & 10.00         & 6.00          & 8.00          & 6.00          & 0.00        & 0.00        & 10.00         & 6.00          & 0.00         & 0.00         & 8.00         & 0.00        \\
                                 & P@5             & 6.00          & 4.80          & 6.80          & 6.80          & 1.60        & 1.60        & 7.20          & 6.00          & 0.00         & 0.00         & 4.80         & 0.40        \\
                                 & mAP             & 9.61          & 9.62          & 10.80         & 10.16         & 3.10        & 3.22        & 11.48         & 10.22         & 2.44         & 2.47         & 8.52         & 2.98        \\ \midrule
\multirow{3}{*}{\textbf{ALL}}    & P@1             & 13.17         & 13.17         & 17.08         & 15.30         & 0.36        & 0.36        & 13.17         & 16.01         & 0.36         & 0.36         & 9.25         & 7.47        \\
                                 & P@5             & 7.12          & 6.12          & 7.97          & 7.90          & 3.35        & 3.35        & 6.90          & 7.19          & 0.50         & 0.50         & 4.70         & 2.78        \\
                                 & mAP             & 15.37         & 14.88         & 18.29         & 17.59         & 4.34        & 4.46        & 14.22         & 15.74         & 3.57         & 3.57         & 10.20        & 7.97        \\ \bottomrule
\end{tabular}
\caption{Probing Results Based on an English Prompt Without Cultural Origin Reference}
\label{tab:en_without}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table*}[ht]
% \centering
% \begin{tabular}{@{}llrrrrrrrrrrrr@{}}
% \toprule
% \textbf{Origin}                  & \textbf{Metric} & \textbf{Bb-c} & \textbf{Bb-u} & \textbf{Bl-c} & \textbf{Bl-u} & \textbf{Rb} & \textbf{Rl} & \textbf{mB-c} & \textbf{mB-u} & \textbf{XRb} & \textbf{XRl} & \textbf{mT5} & \textbf{T5} \\ \midrule
% \multirow{3}{*}{\textbf{U.S.}}   & P@1             & 29.41         & 23.53         & 20.59         & 26.47         & 0.00        & 0.00        & 14.71         & 20.59         & 0.00         & 0.00         & 8.82         & 14.71       \\
%                                  & P@5             & 14.12         & 11.18         & 11.76         & 10.59         & 2.94        & 2.94        & 5.88          & 12.94         & 2.35         & 2.35         & 4.71         & 4.12        \\
%                                  & mAP             & 31.01         & 24.84         & 25.32         & 26.62         & 3.34        & 3.15        & 14.96         & 20.52         & 4.56         & 4.54         & 11.89        & 12.66       \\ \midrule
% \multirow{3}{*}{\textbf{France}} & P@1             & 4.84          & 9.68          & 14.52         & 14.52         & 0.00        & 0.00        & 12.90         & 14.52         & 0.00         & 0.00         & 6.45         & 9.68        \\
%                                  & P@5             & 2.90          & 3.87          & 5.48          & 5.16          & 6.45        & 6.45        & 5.48          & 4.52          & 0.00         & 0.00         & 3.23         & 2.90        \\
%                                  & mAP             & 8.33          & 9.61          & 14.77         & 11.88         & 5.34        & 5.29        & 11.05         & 10.76         & 3.85         & 3.83         & 6.84         & 6.86        \\ \midrule
% \multirow{3}{*}{\textbf{Italy}}  & P@1             & 5.13          & 7.69          & 10.26         & 7.69          & 0.00        & 0.00        & 7.69          & 10.26         & 0.00         & 0.00         & 12.82        & 2.56        \\
%                                  & P@5             & 5.64          & 3.08          & 5.64          & 2.56          & 4.10        & 4.10        & 6.67          & 6.15          & 0.00         & 0.00         & 4.62         & 3.08        \\
%                                  & mAP             & 10.72         & 10.46         & 15.60         & 11.19         & 4.62        & 4.90        & 12.70         & 14.93         & 3.01         & 3.04         & 9.41         & 5.90        \\ \midrule
% \multirow{3}{*}{\textbf{India}}  & P@1             & 23.08         & 23.08         & 23.08         & 7.69          & 0.00        & 0.00        & 7.69          & 23.08         & 0.00         & 0.00         & 7.69         & 7.69        \\
%                                  & P@5             & 7.69          & 6.15          & 7.69          & 7.69          & 1.54        & 1.54        & 6.15          & 7.69          & 0.00         & 0.00         & 6.15         & 4.62        \\
%                                  & mAP             & 29.54         & 26.08         & 30.12         & 20.51         & 2.98        & 2.82        & 17.45         & 29.34         & 1.92         & 2.01         & 18.82        & 11.61       \\ \midrule
% \multirow{3}{*}{\textbf{Japan}}  & P@1             & 10.53         & 10.53         & 10.53         & 5.26          & 5.26        & 5.26        & 21.05         & 15.79         & 5.26         & 5.26         & 0.00         & 0.00        \\
%                                  & P@5             & 5.26          & 5.26          & 6.32          & 6.32          & 1.05        & 1.05        & 5.26          & 5.26          & 1.05         & 1.05         & 3.16         & 1.05        \\
%                                  & mAP             & 12.59         & 12.62         & 12.20         & 11.83         & 7.61        & 7.86        & 16.05         & 12.60         & 6.52         & 6.66         & 5.14         & 2.60        \\ \midrule
% \multirow{3}{*}{\textbf{U.K.}}   & P@1             & 40.00         & 33.33         & 40.00         & 53.33         & 0.00        & 0.00        & 40.00         & 26.67         & 0.00         & 0.00         & 20.00        & 20.00       \\
%                                  & P@5             & 16.00         & 13.33         & 16.00         & 16.00         & 6.67        & 6.67        & 12.00         & 14.67         & 1.33         & 1.33         & 8.00         & 8.00        \\
%                                  & mAP             & 33.52         & 33.58         & 35.24         & 45.35         & 8.44        & 8.51        & 30.84         & 30.70         & 7.53         & 7.46         & 27.68        & 24.10       \\ \midrule
% \multirow{3}{*}{\textbf{Spain}}  & P@1             & 10.00         & 0.00          & 10.00         & 20.00         & 0.00        & 0.00        & 20.00         & 20.00         & 0.00         & 0.00         & 0.00         & 10.00       \\
%                                  & P@5             & 6.00          & 8.00          & 8.00          & 8.00          & 4.00        & 4.00        & 14.00         & 8.00          & 0.00         & 0.00         & 6.00         & 4.00        \\
%                                  & mAP             & 12.33         & 13.36         & 23.08         & 27.33         & 3.48        & 3.77        & 20.84         & 24.05         & 3.13         & 3.17         & 5.34         & 12.16       \\ \midrule
% \multirow{3}{*}{\textbf{China}}  & P@1             & 11.11         & 0.00          & 0.00          & 11.11         & 0.00        & 0.00        & 11.11         & 0.00          & 0.00         & 0.00         & 0.00         & 0.00        \\
%                                  & P@5             & 8.89          & 6.67          & 6.67          & 13.33         & 0.00        & 0.00        & 6.67          & 4.44          & 0.00         & 0.00         & 4.44         & 2.22        \\
%                                  & mAP             & 17.54         & 14.56         & 13.61         & 22.97         & 2.59        & 2.92        & 16.27         & 5.69          & 1.07         & 0.95         & 6.57         & 3.64        \\ \midrule
% \multirow{3}{*}{\textbf{Turkey}} & P@1             & 29.41         & 23.53         & 23.53         & 5.88          & 0.00        & 0.00        & 29.41         & 17.65         & 0.00         & 0.00         & 11.76        & 5.88        \\
%                                  & P@5             & 7.06          & 8.24          & 8.24          & 8.24          & 0.00        & 0.00        & 9.41          & 10.59         & 0.00         & 0.00         & 5.88         & 3.53        \\
%                                  & mAP             & 21.06         & 20.25         & 19.85         & 13.72         & 2.81        & 2.74        & 23.12         & 24.26         & 1.87         & 1.88         & 11.91        & 9.75        \\ \midrule
% \multirow{3}{*}{\textbf{Mexico}} & P@1             & 0.00          & 7.69          & 23.08         & 15.38         & 0.00        & 0.00        & 15.38         & 0.00          & 0.00         & 0.00         & 7.69         & 15.38       \\
%                                  & P@5             & 7.69          & 9.23          & 6.15          & 10.77         & 1.54        & 1.54        & 4.62          & 6.15          & 1.54         & 1.54         & 3.08         & 3.08        \\
%                                  & mAP             & 13.75         & 16.88         & 19.88         & 25.74         & 2.66        & 3.67        & 9.91          & 8.43          & 2.58         & 2.63         & 5.64         & 11.54       \\ \midrule
% \multirow{3}{*}{\textbf{Others}} & P@1             & 12.00         & 12.00         & 10.00         & 8.00          & 0.00        & 0.00        & 10.00         & 8.00          & 0.00         & 0.00         & 8.00         & 2.00        \\
%                                  & P@5             & 6.00          & 5.20          & 6.40          & 6.00          & 1.60        & 1.60        & 7.60          & 5.60          & 0.00         & 0.00         & 4.80         & 0.80        \\
%                                  & mAP             & 10.32         & 10.01         & 11.01         & 9.86          & 3.10        & 3.20        & 10.74         & 9.94          & 2.41         & 2.44         & 8.07         & 3.34        \\ \midrule
% \multirow{3}{*}{\textbf{ALL}}    & P@1             & 13.88         & 13.52         & 15.66         & 14.59         & 0.36        & 0.36        & 14.95         & 13.88         & 0.36         & 0.36         & 8.19         & 7.47        \\
%                                  & P@5             & 7.05          & 6.33          & 7.47          & 7.19          & 3.35        & 3.35        & 6.98          & 7.26          & 0.50         & 0.50         & 4.56         & 2.99        \\
%                                  & mAP             & 15.83         & 15.16         & 17.92         & 17.05         & 4.38        & 4.47        & 14.58         & 15.44         & 3.56         & 3.57         & 9.77         & 8.13        \\ \bottomrule
% \end{tabular}
% \caption{Probing Results Based on an English Prompt With Cultural Origin Reference}
% \label{tab:en_with}
% \end{table*}

==> table/training_corpus.tex <==
\begin{table}[]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{l|l}
    \toprule
    \textbf{Language models}    & \textbf{Training corpus}  \\
    \midrule
    BERT\small~\cite{devlin-etal-2019-bert}        &  BooksCorpus; English Wikipedia \\
    RoBERTa\small~\cite{liu2019roberta}     & BookCorpus; CC-News; OpenWebText\\
    mBERT \small~\cite{devlin-etal-2019-bert}        &  104 languages from Wikipedia \\
    XLM-R\small~\cite{conneau-etal-2020-unsupervised}   & 100 languages from Common Crawl (CCNet)) \\
    T5\small~\cite{JMLR:v21:20-074}  & Common Crawl (C4)  \\
    mT5\small~\cite{xue-etal-2021-mt5} & 101 languages from Common Crawl (mC4)   \\
    \bottomrule
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
    
\end{table}





